STING-BEE: Towards Vision-Language Model for Real-World X-ray Baggage Security Inspection

Advancements in Computer-Aided Screening (CAS) systems are essential for improving the detection of security threats in X-ray baggage scans. However, current datasets are limited in representing real-world, sophisticated threats and concealment tactics, and existing approaches are constrained by a closed-set paradigm with predefined labels. To address these challenges, we introduce STCray, the first multimodal X-ray baggage security dataset, comprising 46,642 image-caption paired scans across 21 threat categories, generated using an X-ray scanner for airport security. STCray is meticulously developed with our specialized protocol that ensures domain-aware, coherent captions, that lead to the multi-modal instruction following data in X-ray baggage security. This allows us to train a domain-aware visual AI assistant named STING-BEE that supports a range of vision-language tasks, including scene comprehension, referring threat localization, visual grounding, and visual question answering (VQA), establishing novel baselines for multi-modal learning in X-ray baggage security. Further, STING-BEE shows state-of-the-art generalization in cross-domain settings. Code, data, and models are available at https://divs1159.github.io/STING-BEE/.

==> Tables/Augmentation_algo.tex <==
\begin{algorithm}
\SetAlgoLined
\DontPrintSemicolon
\caption{Proposed Data Augmentation Approach}
\textbf{Input:} CT volume of threat $C$, X-ray baggage scan $X$, step sizes $\Delta \alpha, \Delta \beta, \Delta \gamma$.\\
\textbf{Output:} X-ray scan with projected threat $X_{out}$

\BlankLine
\ForEach{$\theta_x \in \{0, \Delta \alpha, 2\Delta \alpha, \ldots, 360^\circ\}$}{
    \ForEach{$\theta_y \in \{0, \Delta \beta, 2\Delta \beta, \ldots, 360^\circ\}$}{
        \ForEach{$\theta_z \in \{0, \Delta \gamma, 2\Delta \gamma, \ldots, 360^\circ\}$}{
            $C \gets \text{Rotate}(C, \theta_x, \theta_y, \theta_z)$;\\
            $P \gets$ Integrate $C$ along the Z-axis to yield 2D projection;\\
            Rescale and calibrate $P$ to match the X-ray baggage scan;\\
            $(P_x, P_y) \gets$ Get spatial dimension of $P$;\\
            Select X-ray scan region $S$ for projection with area $(P_x, P_y)$;\\
            Convert the selected area $S$ to grayscale;\\
            $X_t \gets \text{Insert}(P, X, S)$;\\
            $X_{out} \gets \text{Colorize}(X_t)$;\\
            Save $X_{out}$;
        }
    }
}
\label{tab_Augmentation_algo}
\end{algorithm}

==> Tables/tab_Ablation_stages_performance.tex <==

\begin{table}[t!]
    \centering \small
    \caption{\textbf{Ablation :}Impact of training stages and data augmentation on Classification and detection performance.}
    \vspace{-1em}
    \setlength{\tabcolsep}{10pt}
    \scalebox{0.9}[0.9]{
    \begin{tabular}{lcc}
        \toprule
        \rowcolor{Gray} 
        Stage & \makecell{Classification \\ (F1 Score)} & \makecell{Detection \\ (Acc@25)} \\
        \midrule
        First Stage & 12.01 & 9.1 \\
        %\midrule
        Second Stage (without augmentation) & 13.76 & 13.8 \\ 
        \rowcolor{LightCyan}
        Second Stage (with augmentation) & \textbf{14.09} & \textbf{15.4} \\
        \bottomrule
    \end{tabular}%
    }
    \label{tab_Ablation_stages_performance}
    %\vspace{-1.5em}
\end{table}






==> Tables/tab_classification_supervised.tex <==
% \begin{table}[ht!]
%     \centering
%     \caption{Benchmark Results for Various Models}
%     \resizebox{0.7\linewidth}{!}{%
%     \begin{tabular}{@{}lcc@{}}
%         \toprule
%         \textbf{Model} & \textbf{F1 Score} & \textbf{mAP} \\
%         \midrule
%         ResNet50 \cite{resnet} & 5.27 & 6.21 \\
%         EfficientNet-B4 \cite{tan2019efficientnet} & 5.49 & 6.04 \\
%         ViT-B \cite{dosovitskiy2021an} & 3.30 & 6.66 \\
%         DeiT-B \cite{touvron2021training} & 3.22 & 6.72 \\
%         CLIP-ViT-B \cite{Clip_radford} & 4.82 & 6.84 \\
%         LongCLIP \cite{li2022longclip} & 4.61 & 7.71 \\
%         STING BEE & \textbf{14.09} & \textbf{13.52} \\
%         \bottomrule
%     \end{tabular}}
%     \label{tab:classification_supervised}
% \end{table}
\begin{table}[t!]
    \centering \small
    \caption{\textbf{Benchmark Results: }Multi-Label Classification. STING BEE (Proposed) surpasses SOTA methods.}
    \vspace{-1em}
    \centering
    \setlength{\tabcolsep}{20pt}
    \scalebox{0.8}[0.8]{
    \begin{tabular}{lcc}
        \toprule
        \rowcolor{Gray} 
        Model & F1 Score & mAP \\
        \midrule
        ResNet50 \cite{resnet} & 5.27 & 6.21 \\
        EfficientNet-B4 \cite{tan2019efficientnet} & 5.49 & 6.04 \\
        ViT-B \cite{vit} & 3.30 & 6.66 \\
        DeiT-B \cite{touvron2021training} & 3.22 & 6.72 \\
        CLIP-ViT-B \cite{Clip_radford} & 4.82 & 6.84 \\
        LongCLIP \cite{li2022longclip} & 4.61 & 7.71 \\
        \midrule
        \rowcolor{LightCyan}
        STING BEE (Ours) & \textbf{14.09} & \textbf{13.52} \\
        \bottomrule
    \end{tabular}%
    }
    \label{tab_classification_supervised}
    %\vspace{-1.5em}
\end{table}




==> Tables/tab_instance_distribution.tex <==
\begin{table}[b!]
    \centering
    \caption{Statistical distribution of images containing single and multiple threat instances in our dataset}
    \label{tab_instance_distribution}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{lrr}
        \toprule
        \textbf{Mode} & \textbf{Single-Instance Threat Images} & \textbf{Multi-Instance Threat Images} \\
        \midrule
        Train & 23,622 & 5,822 \\
        Test & 12,816 & 3,433\\
        \midrule
        \textbf{Total} & \textbf{36,438} & \textbf{9,255} \\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> Tables/tab_rebuttal_GPT4_LLav_Finetune.tex <==

\begin{table}[t]
\centering
\caption{\scriptsize Our STING-BEE outperforms LLaVa (Finetuned) and GPT-4o. %IL:Instance Location, CR:Complex Reasoning, IID:Instance Identity, IC:Instance Counting, M:Misleading, IA:Instance Attribute, II:Instance Interaction.
}
\vspace{-1em}
\setlength{\tabcolsep}{1.5pt}
\scalebox{0.6}[0.6]{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\rowcolor{Gray}
\textbf{Model} & \multicolumn{2}{c}{\textbf{Scene Comprehension}} & \multicolumn{8}{c}{\textbf{Visual Question Answering}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-11} 
               & F1   & mAP  & IL & CR & IID & IC & M & IA & II & Overall  \\ \midrule

LLaVa 1.5 (Finetuned)&28.3& 22.2 & 35.2 & 59.4 & 77.8 &36.1& 15.9 & 48.2 &  25.3 & 45.1    \\
GPT-4o& 19.4  & 18.1  &  21.5   &  16.2    &  36.3  &  29.6   &  25.2  & 19.02  &   18.3   &   31.3  \\ \midrule
STING-BEE&\textbf{34.7}& \textbf{29.8} & \textbf{49.2} & \textbf{79.2} & \textbf{80.0}  &  \textbf{45.2} & \textbf{27.8} & \textbf{52.8} & \textbf{35.0}  & \textbf{52.8} \\ 
\bottomrule
\end{tabular}
}
\label{tab_rebuttal_GPT4_LLav_Finetune}
\vspace{-2em}
\end{table}


% \begin{table*}[t]
% \centering
% \caption{Performance comparison with STING-BEE on Cross-domain Scene Comprehension and  VQA.}
% \vspace{-1em}
% \setlength{\tabcolsep}{6pt}
% \scalebox{0.75}[0.75]{
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
% \rowcolor{Gray}
% \textbf{Model} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Cross-domain Scene \\ Comprehension\end{tabular}}} & \multicolumn{8}{c}{\textbf{Visual Question Answering}} \\ 
% \cmidrule(lr){2-3} \cmidrule(lr){4-11} 
%                & F1& mAP& Instance Location&Complex Reasoning& Instance Identity&Instance Counting & Misleading & Instance Attribute&Instance Interaction&Overall\\ \midrule

% LLaVa 1.5 (Finetuned)&   &     &     &      &     &     &    &   &      &     \\
% GPT-4o&   &     &     &      &     &     &    &   &      &      \\

% STING-BEE&34.69& 29.80 & 49.22 & 79.21 & 80.04  &  45.24 & 27.76 & 52.85 & 35.03  & 52.81 \\ 
% \bottomrule
% \end{tabular}
% }
% \label{tab:rebuttal_GPT4_LLav_Finetune}
% \vspace{-1em}
% \end{table*}




==> Tables/tab_rebuttal_Qwen_Llama_STINGlimited.tex <==

\begin{table}[t]
\centering
\caption{\scriptsize Our STING-BEE outperforms Llama 3.2 and Qwen2-VL. IL:Instance Location, CR:Complex Reasoning, IID:Instance Identity, IC:Instance Counting, M:Misleading, IA:Instance Attribute, II:Instance Interaction.
}
\vspace{-1em}
\setlength{\tabcolsep}{1.8pt}
\scalebox{0.5}[0.5]{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\rowcolor{Gray}.
\textbf{Model} & \multicolumn{2}{c}{\textbf{Scene Comprehension}} & \multicolumn{8}{c}{\textbf{Visual Question Answering (VQA)}} & \multicolumn{2}{c}{\textbf{Grounding}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-11} \cmidrule(lr){12-13}
               & F1   & mAP  & IL & CR & IID & IC & M & IA & II & Overall & acc@0.5 & acc@0.25 \\ \midrule
Llama 3.2 & 13.4 & 17.3 &  26.5 &  29.3 &  36.3 &   20.8 &  11.6&   25.4 &  13.3 &  23.5 & 1.9 &5.3\\ 
Qwen2-VL&18.6&16.9&31.3&15.1&41.3&24.1&18.8&36.1&13.1&27.8&1.2&3.9\\
\begin{tabular}[l]{@{}l@{}}STING-BEE \\(limited captions)\end{tabular}&22.1&18.2&25.3&41.3&69.2&35.4&20.5&42.2&27.6&41.8&5.3&14.1\\
\midrule
STING-BEE&\textbf{34.7}& \textbf{29.8} & \textbf{49.2} & \textbf{79.2} & \textbf{80.0}  &  \textbf{45.2} & \textbf{27.8} & \textbf{52.8} & \textbf{35.0}  & \textbf{52.8}&\textbf{8.7}&\textbf{21.5} \\ 
\bottomrule
\end{tabular}
}
\label{tab_rebuttal_Qwen_Llama_STINGlimited}
\vspace{-1em}
\end{table}







% \begin{table*}[t]
% \centering
% \caption{Performance comparison with STING-BEE on Scene Comprehension, Visual Question Answering, and Grounding tasks.}
% \vspace{-1em}
% \setlength{\tabcolsep}{6pt}
% \scalebox{0.75}[0.75]{
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
% \rowcolor{Gray}
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Scene Comprehension}} & \multicolumn{8}{c}{\textbf{Visual Question Answering}} & \multicolumn{2}{c}{\textbf{Grounding}} \\ 
% \cmidrule(lr){2-3} \cmidrule(lr){4-11} \cmidrule(lr){12-13}
%                & F1   & mAP  & \begin{tabular}[c]{@{}c@{}}Instance \\ Location\end{tabular} & \begin{tabular}[c]{@{}c@{}}Complex \\ Reasoning\end{tabular} & \begin{tabular}[c]{@{}c@{}}Instance \\ Identity\end{tabular} & \begin{tabular}[c]{@{}c@{}}Instance \\ Counting\end{tabular} & Misleading & \begin{tabular}[c]{@{}c@{}}Instance \\ Attribute\end{tabular} & \begin{tabular}[c]{@{}c@{}}Instance \\ Interaction\end{tabular} & Overall & acc@0.5 & acc@0.25 \\ \midrule
% Llama 3.2 & 13.41 & 17.32 &  26.51 &  29.25 &  36.30 &   20.79 &  11.61&   25.4 &  13.26 &  23.53 & 1.9 &5.3\\ 
% Qwen2-VL&18.55&16.87&31.29&15.12&41.27&24.14&18.75&36.12&13.14&27.82&1.2&3.9\\
% \begin{tabular}[c]{@{}c@{}}STING-BEE \\(limited)\end{tabular}&22.13&18.17&25.27&41.29&69.18&35.38&20.47&42.19&27.59&41.84&5.3&14.1\\
% \midrule
% STING-BEE&34.69& 29.80 & 49.22 & 79.21 & 80.04  &  45.24 & 27.76 & 52.85 & 35.03  & 52.81&8.7&21.5 \\ 
% \bottomrule
% \end{tabular}
% }
% \label{tab:rebuttal_Qwen_Llama_STINGlimited}
% \vspace{-1em}
% \end{table*}





==> Tables/tab_supervised_detection.tex <==
\begin{table}[t!]
    \centering \small
    \caption{\textbf{Benchmark Results :}Threat Detection. Performance across SOTA methods, evaluated using AP and AP@50.}
   \vspace{-1em}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{llc}
        \toprule
        \rowcolor{Gray} 
        \textbf{Model Category} & \textbf{Model} & \textbf{AP / AP@50} \\
        \midrule
        \multirow{5}{*}{\textbf{Specialist Models}} 
        & Faster RCNN \cite{ren2017faster} & 9.93 / 16.69 \\
        & Cascaded RCNN \cite{cai2018cascade} & 11.58 / 20.33 \\
        & GDINO \cite{liu2024groundingdino} & 17.40 / 22.10 \\
        & DETR \cite{carion2020detr} & 8.50 / 13.30 \\
        & YOLOv11 \cite{yolov11} & 17.30 / 22.80 \\
        \midrule
        \multirow{2}{*}{\textbf{Specialist X-ray Models}} 
        & SDANet \cite{pidray} & 19.40 / 28.30 \\
        & TPD \cite{hassan2022tensor} & 17.41 / 25.81 \\
        \midrule
        \rowcolor{LightCyan}
        \textbf{Ours} & STING BEE & 6.14 / 10.91 \\
        \bottomrule
    \end{tabular}}
    \label{tab_supervised_detection}
    %\vspace{-1.5em}
\end{table}







==> Tables/threat_instances.tex <==
\begin{table}[ht]
    \centering \small
    \caption{Instance-wise distribution of threat items in STCray Dataset}
    \vspace{-1em}
    \centering
      \setlength{\tabcolsep}{16pt}
    % \scalebox{0.8}[0.8]{
    \begin{tabular}{lc}
        % \centering \small
        \toprule
        \textbf{Category} & \textbf{Number of Instances} \\
        \midrule
        Explosive & 4 \\
        Gun & 6  \\
        3D Printed Gun & 3  \\
        Knife & 4\\
        Cutter & 5	\\
        Blade & 1\\
        Shaving Razor &4  \\
        Lighter & 6 \\
        Syringe & 2	\\
        Battery & 4  \\
        Nail Cutter & 2 \\
        Other Sharp Items & 3	 \\
        Powerbank & 4 \\
        Scissors & 4 \\
        Hammer & 4\\
        Pliers & 5	 \\
        Wrench & 3	\\
        Screwdriver & 4	\\
        Handcuffs & 2	\\
        Bullet & 5  \\
        \midrule
        \textbf{Total} & \textbf{75}  \\ % Bolded total line
        \bottomrule
    \end{tabular}%
    % }
    \label{tab_threat_instances}
    \vspace{-1.5em}
\end{table}
